Functional Expansions

Path dependence is omnipresent in many disciplines such as engineering, system theory and finance. It reflects the influence of the past on the future, often expressed through functionals. However, non-Markovian problems are often infinite-dimensional, thus challenging from a conceptual and computational perspective. In this work, we shed light on expansions of functionals. First, we treat static expansions made around paths of fixed length and propose a generalization of the Wiener series$-$the intrinsic value expansion (IVE). In the dynamic case, we revisit the functional Taylor expansion (FTE). The latter connects the functional It\^o calculus with the signature to quantify the effect in a functional when a "perturbation" path is concatenated with the source path. In particular, the FTE elegantly separates the functional from future trajectories. The notions of real analyticity and radius of convergence are also extended to the path space. We discuss other dynamic expansions arising from Hilbert projections and the Wiener chaos, and finally show financial applications of the FTE to the pricing and hedging of exotic contingent claims.

==> Dynamic/JunkChaos.tex <==
\underline{\textbf{Wiener Chaos  (\cref{sec:chaos}).}} Establishing a parallel between the FTE and Wiener chaos expansions proves 
simple in specific cases. In this section, we restrict ourselves to  non-exotic   payoffs $g(X_T)=h(x_T)$, with $h: \R \to \R$. On the other hand, we momentarily allow $\Q$ to be any measure such that $X$ is an $(\F,\Q)-$Markov process. This implies that the price functional $f(X_t) =\E^{\Q}[g(Y_T)\,|\,X_t]$, seen in \cref{ex:pricefunctional}, is function of $x_t$ only.  
We begin with a trivial yet important lemma. In the sequel, let $X^{t,x}$ be the path  on $[t,T]$ such that $x_t^{t,x}=x$ and denote by $ \nabla{X}^{t,x}$ its \textit{ tangent}  (or \textit{first variation}) \textit{process}  \cite{IkedaWatanabe,DiNunno}, 
 $$ \nabla {x}_s^{t,x} = \lim_{\delta x \to 0} \frac{x_s^{t,x+\delta x}-x_s^{t,x}}{\delta x}, \quad s \in [t,T],$$
 when the above is well-defined. 
 The tangent process measures the effect of an instantaneous shock on a path at later dates. For example, if $\Q$ is the law of an Ornstein-Uhlenbeck process with unit mean reversion speed,  
 then $\nabla{x}_s^{t,x} = e^{-(s-t)}$, i.e., the impact of a bump 
 decays exponentially.

\begin{lemma}\label{lem:Tangent}
Let $X$ be an $(\F,\Q)-$Markov process with bounded tangent process and $g(X_T)=h(x_T)$ for some $h\in \calC_b^{1}(\R)$. If $f(X_t) = \E^{\Q}[g(Y_T)\,|\,X_t]$, then
  $\Delta_{x}f(X_t) = \E^{\Q}[\Delta_{x}g(Y^{t,x}_T) \, \nabla y^{t,x}_T 
  ]\big |_{x=x_t}.$
\end{lemma}

\begin{proof} This simply follows from the chain rule and the bounded convergence theorem. 
\end{proof}
More can be said when $X$ has unit tangent process, namely $\nabla{X}^{t,x}  \equiv 1$. We describe such process as \textit{arithmetic}. An example in finance is the underlying in the Bachelier model. 
In this case, $X$ is actually an arithmetic Brownian motion, 
 whence the terminology. 
The following result provides a characterization of path independence for $T-$functionals. % and  brings us one step closer to a  connection between the FTE and Wiener chaos expansion. 
\begin{proposition}\label{prop:Martingale}
Let 
$f(X_t) = \E^{\Q}[g(Y_T)\,|\,X_t]$ for a   $T-$functional $g$ such that $\calA_T g \in \calD_{\calA}$.  Then the following are equivalent: 
\begin{itemize}
\item[(i)] $g$ is path-independent. 
\item[(ii)]  $\Delta_{\mathds{1}_k} f(X)$ is an $(\Q,\F)-$martingale for all $k\ge 0$. 
\item[(iii)]  The Wiener chaos expansion writes $g(X_T) = \sum_{k=0}^{\infty}\Delta_{\mathds{1}_k}f(\boldsymbol{0}) J_k(X_T)$.
\end{itemize}
\end{proposition}

\begin{proof}
See \cref{app:Martingale}.
\end{proof}

In derivatives pricing, 
$X$ has to be interpreted as the source of risk, which usually differs from the underlying.  
For instance, a call option in the Black-Scholes with zero dividend and interest rate would read $g(X_T) = (\calI(X_T) -K)^+$, where $X$ is Brownian motion and $\calI$  the  It\^o map $\calI(X_T) = x_0 e^{\sigma x_T - \frac{1}{2}\sigma^2T}$.
Exceptions include the Bachelier model, where $X$  is the asset itself. In this case, the spatial derivatives correspond to the option Delta, Gamma, and so on.

\begin{corollary}
Under the assumptions of  \Cref{prop:Martingale} and supposing that $g$ is path-independent, then the functional Wiener-Itô chaos expansion of $f$ writes
$f(X_t) = \sum_{k=0}^{\infty}\Delta_{\mathds{1}_k}f(\boldsymbol{0}) J_k(X_t).$
\end{corollary}

\begin{proof}
Take conditional expectation in  \cref{prop:Martingale} (iii) and use the martingality of $J_k(X)$. 
\end{proof}
Next, we show that the $k-$fold It\^o iterated integrals are linear combinations of finitely many elements of the signature. 
First, we employ the representation
 \begin{equation}\label{eq:Hermite}
    J_{k}(X_t) = h_k(t,x_t), \quad  h_k(t,x) =  \frac{t^{k/2}}{k!}H_k\left(\frac{x}{\sqrt{t}}\right),  
 \end{equation}
where $H_k$ is the $k-$th probabilist's Hermite polynomial; see  \cite{DiNunno}. 
Although the process $J_k(X)$ is indistinguishable from $h_k(\cdot,x)$, their functional derivatives may differ as nicely 
explained by \citet{Oberhauser}. 
However, using the functional It\^o formula and the uniqueness of the  Doob-Meyer decomposition, the operator $\calL := \Delta_t +  \frac{1}{2}\Delta_{xx},$ must act in the same way,  regardless of the representation chosen; see again 
\cite{Oberhauser}. 
For obvious reasons, $\calL$ is often called the   \textit{causal}  \textit{heat operator}. %\textit{functional}
The next simple lemma relates the It\^o iterated integrals to the signature. 

\begin{lemma}\label{lem:hermite}
The It\^o iterated integrals are smooth functionals and admit the Maclaurin expansions 
  \begin{align*}
      J_{k}(X_t)
      = \sum_{\alpha \in \A_k} (-2)^{-|\alpha|_0}  \calS_{\alpha}(X_t),  \quad k \ge 0,
 \end{align*}
with  the disjoint subsets 
 $\A_k = \left\{\alpha \in \A \ : \ \lVert \alpha\rVert = k \right\}$, $\ \lVert \alpha\rVert := 2|\alpha|_0 + |\alpha|_1$. 
\end{lemma}

\begin{proof} See \cref{app:hermite}.
\end{proof}
We observe from \cref{lem:hermite} that  It\^o iterated integrals induce a partition of the words in $\A$ 
based on the "weighted length" $\lVert \cdot \rVert$. Note that the  latter arises naturally when establishing convergence results about iterated It\^o or Stratonovich integrals  \cite{KP,BenArous,LyonsVictoir}. 
Finally, we bridge the gap between the FTE and Wiener-It\^o chaos expansion in this simple case. 
\begin{proposition}\label{prop:connectionIndep}
Let $g$ be a bounded, analytic path-independent $T-$functional and $f(X_t) = \E^{\Q}[g(Y_T)\,|\,X_t]$.  Under the assumptions of  \Cref{prop:Martingale}, then $\Delta_{\mathds{1}_k} f(\boldsymbol{0}) (-2)^{-|\alpha|_0}=\Delta_{\alpha}f(\boldsymbol{0}) $ and in turn, 
   \begin{equation*}
       g(X_T) = \sum_{k=0}^{\infty} J_k \phi_k(X_T)  = \sum_{k=0}^{\infty} \sum_{\alpha \in \A_k} \Delta_{\mathds{1}_k} f(\boldsymbol{0}) (-2)^{-|\alpha|_0}   \calS_{\alpha}(X_T) = \sum_{\alpha }
   \Delta_{\alpha}f(\boldsymbol{0})    \calS_{\alpha}(X_T).
   \end{equation*}
\end{proposition} 

\begin{proof} 
As $g$ is path-independent, 
\cref{prop:Martingale} gives
$
g(X_T) = 
\sum_{k=0}^{\infty}\Delta_{\mathds{1}_k}f(\boldsymbol{0}) J_k(X_T)
$ and  $\Delta_{\mathds{1}_k} f(X)$ is a $(\Q,\F)-$ martingale for all $k\ge 0$. As $X$ is Brownian motion, the functional It\^o formula \cite{Dupire} implies that each $\Delta_{\mathds{1}_k} f$ solves  the path-dependent PDE  
$\calL \varphi =  \left(\Delta_t + \frac{1}{2}\Delta_{xx} \right)\varphi=0.$ 
Put differently, any second spatial derivative can be converted into a temporal derivative by multiplying by the factor $-2$. Thus,  $\Delta_{\mathds{1}_k}f =  (-2)^{|\alpha|_0} \ \Delta_{\alpha} f$ for every word $\alpha \in \A_k$. 
   Together with \cref{lem:Tangent}, the result follows. 
\end{proof}
\begin{remark}
In the general case where the kernels are time-dependent 
it is delicate to compare the Wiener chaos expansion with the FTE. Indeed, we would need to expand the terms $J_k \phi_k$ which does not have the required regularity if expressed pathwise;  
see the discussion in \cite{Oberhauser}. Inversely, one can compute the Wiener chaos expansion of each signature functional, namely $\calS_{\alpha}(X_T) = \sum_{k=0}^{\infty} J_k \phi_k(X_T)$ for some  kernels  $(\phi_k)$ to be determined. In light of Stroock's formula $\eqref{eq:stroock}$, one has to compute the expected higher-order Malliavin derivatives of the signature to obtain $(\phi_k)$. 
This was conducted recently by \citet{Cass} for a wide class of Gaussian processes encompassing fractional Brownian motion %(fBm) 
with Hurst parameter $H\in(1/4,1)$. More precisely, the kernels $(\phi_k)$ are expressed in terms of the covariance function of $X$. 
\end{remark}
